HammerHead: Leader Reputation for Dynamic Scheduling

The need for high throughput and censorship resistance in blockchain technology has led to research on DAG-based consensus. The Sui blockchain protocol uses a variant of the Bullshark consensus algorithm due to its lower latency, but this leader-based protocol causes performance issues when candidate leaders crash. In this paper, we explore the ideas pioneered by Carousel on providing Leader-Utilization and present HammerHead. Unlike Carousel, which is built with a chained and pipelined consensus protocol in mind, HammerHead does not need to worry about chain quality as it is directly provided by the DAG, but needs to make sure that even though validators might commit blocks in different views the safety and liveness is preserved. Our implementation of HammerHead shows a slight performance increase in a faultless setting, and a drastic 2x latency reduction and up to 40% throughput increase when suffering faults (100 validators, 33 faults).

==> Graveyard.tex <==

From Chapter 3:

% \paragraph{Things to prove.} We would like to prove that our extension protocol satisfies (maintains or adds) the following properties:
% \begin{enumerate}
%     \item Safety: Every validator computes the same leader schedule. This implies safety (assuming that Bullshark is safe).
%     \item Liveness: After GST, honest validators are eventually elected as leaders. This implies liveness (assuming that Bullshark is live).
%     \item Fairness: After GST, all honest validators have an equal chance of being elected leaders. (Lemma: All honest validators are part of the set Q). \giorgos{We need liveness for that.}
%     \item Efficiency 1: After GST, honest validators are elected more often than crashed validators. \giorgos{Liveness}
%     \item Efficiency 2 (optional): After GST, Crashed validators are elected as leaders at most L times (where L is bounded and/or small).\giorgos{Liveness}
%     \item Redeemability: Validators who crashed and recovered have the opportunity to be elected leaders. That is, after GST, an honest validator starting with 0 reputation score is eventually elected as a leader regardless of the scores of other validators. \giorgos{Liveness}
% \end{enumerate}

% The efficiency property is required to avoid the trivial case where reputation scores are never updated and the system runs round-robin forever. That is, the efficiency property demonstrates that we gain something by implementing this protocol rather than the current Bullshark.

%\input{figures/oldCommitExample}


% \begin{proposition}[Integrity]\label{proposition:integrity}
% \sys satisfies Integrity per \emph{BAB}.
% \end{proposition}

% \begin{proof}
%     An honest party $p_i$ outputs $a\_deliver_i(b,r,s)$ if there is a vertex $\mathsf{v}$ in $DAG_i$ such that $(\mathsf{v}.block, \mathsf{v}.round, \mathsf{v}.source) = (b,r,s)$. Since all vertices are reliable broadcast, then by the Integrity of BRB there are no two different vertices $\mathsf{u},\mathsf{u}'$ in $DAG_i$ such that both $\mathsf{u}.round = \mathsf{u}'.round$ and $\mathsf{u}.source= \mathsf{u}'.source$ hold simultaneously.\hfill\qed   
% \end{proof}

==> algorithms/updateSchedule.tex <==
\begin{algorithm}[H]
    \caption{Updating the schedule view of party $p_i$ on round $\mathsf{r}$ where commit occurs.}
    \begin{algorithmic}[1]
        \alglinenoPop{counter}
        \small

        \Statex \textbf{Local variables:}

        \StateX \revisit{$\scores \gets $ initialize empty $1\times n$ table}\giorgos{check where the initialization/view should be}

        \Statex

        \Procedure{\textsc{updateScores}}{$\mathsf{r}, \mathsf{votes}$}
        \For{$\mathsf{v}\in\mathsf{votes}$}
        \State $\scores[\mathsf{v}]+=1$
        \EndFor
        \If{$\mathsf{r}\mod\mathsf{K}==0$}
        \State \textsc{updateSchedule}()
        \State \revisit{\textsc{RetryCommiting}()}
        \giorgos{Simplifying for now, more correct call required}
        \EndIf



        \EndProcedure

        \Statex

        \Procedure{\textsc{updateSchedule}()}{}
        \State $B\leftarrow$ the $k<f$ parties with worst scores in $\scores[\cdot]$
        \State $G\leftarrow$ the $k<f$ parties with best scores in $\scores[\cdot]$
        \For{slot $s\in\mathsf{Schedule}[\cdot] \mid \mathsf{leader}(s)= \mathsf{v}_b\in B$}
        \State \textsc{replace}$(\mathsf{v}_b, G)$
        \EndFor
        \State Reset $\scores[\cdot]$ to $[0,\dots,0]$

        \EndProcedure

        \Statex

        \Procedure{\textsc{replace}}{$\mathsf{v}_b, G$}
        \State $\mathsf{v}_g\tilde{\leftarrow} G$
        \If{$\mathsf{v}_g==\perp$} \Return \EndIf
        \State $T[\mathsf{v}_g,1]+=1;T[\mathsf{v}_b,1]-=1$
        \State Replace $\mathsf{v}_b$ with $\mathsf{v}_g$ in $\mathsf{Schedule}[s]$
        \State \Return

        % \If{$\mathsf{v}_g==\perp$} \Return \EndIf
        % \If{$T[\mathsf{v}_g,0] < 1.5*T[\mathsf{v}_g,1]$} \lef{this was kind of arbitrary for fairness in the notion doc, I would remove it for now}
        % \State $T[\mathsf{v}_g,1]+=1;T[\mathsf{v}_b,1]-=1$
        % \State Replace $\mathsf{v}_b$ with $\mathsf{v}_g$ in $\mathsf{Schedule}[s]$
        % \State \Return
        % \Else
        % \State Remove $\mathsf{v}_g$ from $G$
        % \State \textsc{replace}$(\mathsf{v}_b, G)$
        % \EndIf
        \EndProcedure
        %\eindent

        % \State $X \gets x$
        % \State $N \gets n$
        % \While{$N \neq 0$}
        % \If{$N$ is even}
        %     \State $X \gets X \times X$
        %     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
        % \ElsIf{$N$ is odd}
        %     \State $y \gets y \times X$
        %     \State $N \gets N - 1$
        % \EndIf
        % \EndWhile

    \end{algorithmic}
\end{algorithm}




==> figures/oldCommitExample.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\begin{scope}[every node/.style={circle,thick,draw}]
    \node (A) at (0,0) {$r_0$};
    \node (B) at (3,0) {$r_c$};
    \node (C) at (5,0) {$r_S$};
    \node (D) at (8,0) {$r_{nc}$};
    \node (E) at (11,0) {$r_T$};
\end{scope}



\draw[-edge] (a) -- (b);

% compute a point in the middle between E and NE or W and NW, then draw a line between these two
\path (a.east) -- (a.north east) coordinate[pos=0.5] (a1);
\path (b.west) -- (b.north west) coordinate[pos=0.5] (b1);
\draw[edge-] (a1) -- (b1);




\begin{scope}[>={Stealth[black]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=red,very thick}]
    %\path [->] (C) [dashed] node {} (B);  
    \path [->] (B) edge node {$3$} (C);

    \path [->] (D) edge node {$3$} (C);
    \path [->] (D) edge node {$3$} (E);
    %\path [->] (B) edge[bend right=60] node {$1$} (E); 
\end{scope}

\begin{scope}[dashed]
    \draw (C) -> (B);
`   \draw (D) -> (C);
\end{scope}
\end{tikzpicture}
\caption{A caption.}
\end{figure}

==> sections/liveness.tex <==


\section{Guaranteed Liveness}















==> sections/unresponsive.tex <==
\section{Non-responsive Protocol}

\giorgos{Not worked on it yet, just moved the Notion notes for now.}\\
\paragraph{Proposal Protocol (Non-Responsive).} There is an initial schedule $S$ which is either the classic round-robin or a biased round-robin based on the results of the previous epoch. We keep this schedule for $K$ rounds.
Each validator maintains a data structure mapping each validator to their reputation score; every validator starts with a 0 reputation score.
- Upon committing a sub-dag, the consensus modules update the reputation score of each validator using a deterministic rule. Since all validators observe the same sequence of committed sub-dags, they all attribute the same reputation scores to validators. We propose the following deterministic rule to update reputation scores:
    - Each validator receives 1 point each time they vote for a leader’s proposal. The reputation score of each validator is incremented by the number of points they accumulate.
- After the validator committed K sub-dags (and updated the reputation scores of each validator as described above), they compute a new leaders’ schedule S’.
- Validators reset their map of reputation scores (the reputation score of each validator is set to 0).
- The new schedule takes effect immediately; that is, the (K+1)th committed sub-dag is determined based on the new schedule.

This proposal is not responsive: to prove liveness, every validator needs to wait for the timeout delta before being able to make progress and propose a new rounds. In practice we may not care since we already wait a bit to gather enough batches (and we also have a minimum delay).

Also, we may want to only update the schedule upon committing a leader that is linked to the first committed leader of the new scheduled; this allows us to preserve the safety proof of Bullshark. That is, in the example above, upon committing L1, we only update the schedule if L1 and L2’ are linked.

\paragraph{Questions}

- What are the advantages of using rule 1 (count leader certificates) vs rule 2 (count votes) to update reputations scores? How gamable is each approach?
- What should be a typical value of S? The simplest seems to make S match the duration of an epoch.
- Should we allow validators to appear in the set Q more than once (eg. proportionally to their score)?

% \paragraph{Things to prove}

% 1. Safety: Every validator computes the same leader schedule. This implies safety (assuming Bullshark is safe).
% 2. Liveness: After GST, honest validators are eventually elected as leaders. This implies liveness (assuming Bullshark is live).
% 3. Fairness: After GST, all honest validators have an equal chance to be elected as leaders. (Lemma: all honest validators are part of the set Q).
% 4. Efficiency 1: After GST, honest validators are elected more often than crashed validators.
% 5. Efficiency 2 (optional): After GST, Crashed validators are elected as leaders at most L times (where L is bounded and/or small).
% 6. Mercifulness (better name?): Validators who crashed and recovered have a chance to be elected as leaders. That is, after GST, an honest validator starting with 0 reputation score is eventually elected as a leader regardless of the scores of other validators.

% The efficiency property is required to avoid the trivial case where reputation scores are never updated and the system runs round-robin forever. That is, the efficiency property demonstrates that we gain something by implementing this protocol rather than the current Bullshark.
\label{sec:unresponsive}
